Dataset Distillation for Handwritten Text Recognition: An Empirical Study

Dataset distillation (DD) replaces large training datasets with smaller synthetic ones to reduce computational costs. While traditionally used for classification, we present, to our knowledge, the first DD study for line-level handwritten text recognition (HTR). Unlike classification tasks, which use discrete labels, HTR employs unaligned sequences from a virtually infinite output space as labels. To adapt classification-based DD methods to this scenario, we define text pseudo-classes by clustering transcriptions based on character n-grams. We adapt gradient matching (GM), distribution matching (DM) and trajectory matching (MTT) to a Convolutional Recurrent Neural Network (CRNN) trained with Connectionist Temporal Classification (CTC). In this process, synthetic line images are generated by optimising only the pixels of real starting lines (either randomly chosen or selected as text medoids), while keeping their original transcriptions fixed. Across four datasets (IAM, George Washington, READ\,2016, LAM) and three budgets (1--10\,\% of the training lines), no distilled set outperforms its real initialisation lines. Random lines prove better than medoids, and further optimisation only degrades recognition. Methodologically, DM lowers its objective without benefit, while GM and MTT barely move theirs. We turn these findings into guidelines for evaluating data compression in HTR.

==> tables/supp_objective.tex <==
IAM & 62 & 0.980 [0.979, 0.982] & 0.983 [0.982, 0.984] & 1.000 [1.000, 1.000] & 0.995 [0.994, 0.996] & 1.000 [1.000, 1.000] & 1.002 [1.001, 1.002] \\
IAM & 308 & 0.997 [0.996, 0.997] & 0.997 [0.997, 0.997] & 1.000 [1.000, 1.000] & 0.999 [0.999, 0.999] & 1.000 [1.000, 1.000] & 1.000 [1.000, 1.000] \\
IAM & 616 & 0.998 [0.998, 0.999] & 0.999 [0.999, 0.999] & 1.000 [1.000, 1.000] & 0.999 [0.999, 0.999] & 1.000 [1.000, 1.000] & 1.000 [1.000, 1.000] \\
GW & 4 & 0.704 [0.688, 0.721] & 0.770 [0.762, 0.778] & 0.992 [0.991, 0.993] & 0.969 [0.965, 0.974] & 1.001 [1.001, 1.002] & 0.982 [0.977, 0.986] \\
GW & 18 & 0.917 [0.911, 0.924] & 0.924 [0.922, 0.925] & 0.998 [0.998, 0.999] & 0.994 [0.992, 0.995] & 0.999 [0.999, 0.999] & 0.998 [0.998, 0.999] \\
GW & 36 & 0.948 [0.945, 0.952] & 0.959 [0.958, 0.961] & 0.999 [0.999, 0.999] & 0.993 [0.991, 0.995] & 1.000 [0.999, 1.000] & 1.000 [1.000, 1.000] \\
READ\,2016 & 84 & 0.977 [0.976, 0.979] & 0.975 [0.973, 0.976] & 1.000 [0.999, 1.000] & 0.996 [0.996, 0.997] & 1.000 [1.000, 1.000] & 0.998 [0.998, 0.999] \\
READ\,2016 & 418 & 0.995 [0.994, 0.995] & 0.996 [0.995, 0.996] & 1.000 [1.000, 1.000] & 0.999 [0.999, 0.999] & 1.000 [1.000, 1.000] & 1.000 [1.000, 1.000] \\
READ\,2016 & 835 & 0.997 [0.997, 0.997] & 0.998 [0.998, 0.998] & 1.000 [1.000, 1.000] & 1.000 [0.999, 1.000] & 1.000 [1.000, 1.000] & 1.000 [1.000, 1.000] \\
LAM & 198 & 0.992 [0.991, 0.992] & 0.992 [0.991, 0.993] & 1.000 [1.000, 1.000] & 0.999 [0.998, 0.999] & 1.000 [1.000, 1.000] & 1.000 [1.000, 1.000] \\
LAM & 991 & 0.998 [0.998, 0.998] & 0.998 [0.998, 0.998] & 1.000 [1.000, 1.000] & 1.000 [1.000, 1.000] & 1.000 [1.000, 1.000] & 1.000 [1.000, 1.000] \\
LAM & 1983 & 0.999 [0.999, 0.999] & 0.999 [0.999, 0.999] & 1.000 [1.000, 1.000] & 1.000 [1.000, 1.000] & 1.000 [1.000, 1.000] & 1.000 [1.000, 1.000] \\

